Learning logic programs by discovering higher-order abstractions

We introduce the higher-order refactoring problem, where the goal is to compress a logic program by discovering higher-order abstractions, such as map, filter, and fold. We implement our approach in Stevie, which formulates the refactoring problem as a constraint optimisation problem. Our experiments on multiple domains, including program synthesis and visual reasoning, show that refactoring can improve the learning performance of an inductive logic programming system, specifically improving predictive accuracies by 27% and reducing learning times by 47%. We also show that Stevie can discover abstractions that transfer to multiple domains.

==> framework-OLD.tex <==
\section{Problem Setting}
\label{sec:setting}

We now introduce our problem setting.
% and show how it can improve learning performance.
% \paragraph{Preliminaries.}
We assume familiarity with logic programming \cite{lloyd:book} but have included a summary in the appendix. 
We restate key terminology.
% All sets are finite unless otherwise stated.
A \emph{first-order variable} can be bound to a constant symbol or another first-order variable.
A \emph{higher-order variable} can be bound to a predicate symbol or another higher-order variable.
A \emph{clause} is a set of literals.
% A \emph{rule} is a clause and vice-versa.
We use \emph{rule} synonymously with \emph{clause}.
A clause is \emph{higher-order} if it has at least one higher-order variable.
A program is \emph{higher-order} if it has at least one higher-order clause.
% \ac{and \emph{size} be a function that measures the size of a logic program.}
% A \emph{clausal theory} is a set of clauses.
A \emph{definite clause} is a clause with exactly one positive literal.
A \emph{definite program} is a set of definite clauses.
The \emph{size(P)} of the logic program $P$ is the number of literals in $P$.
A \emph{definition} is a set of clauses with the same head predicate symbol:

\begin{definition}[\textbf{Definition}]
Let $T$ be the set of head predicate symbols in the logic program $P$.
Then the set of definitions of $P$ is
$
D(P) = \bigcup\limits_{p \in T}{\{r \in P | \text{$p$ is the head predicate of the rule $r$}\}}
$  
\end{definition}
% \ac{do we need this as a definition or is the informal description sufficient?}
\noindent
% \ch{shall we consider a logic program and a set of definitions as equivalent? which one should we use?}
% The definitions of a program consist of its rules. These definitions may also be recursive or include predicate invention, in which case a single definition contains multiple rules.


% \subsection{ILP Problem}
% We introduce the ILP problem. We first define an ILP input:

% \begin{definition}[\textbf{ILP input}]
% An ILP input is a tuple $(B,E^+,E^-,{\mathcal{H}})$, where $B$ is a logic program denoting BK, $E^+$ and $E^-$ are sets of ground atoms denoting positive and negative examples respectively, and ${\mathcal{H}}$ is a hypothesis space.
% \end{definition}

% \noindent
% We formulate the ILP problem in the learning from entailment setting \cite{luc:book}:

% \begin{definition}[\textbf{ILP problem}]
% Given an ILP input $(B,E^+,E^-,{\mathcal{H}})$, the ILP problem is to return a hypothesis $h \in \mathcal{H}$ such that
% $\forall e \in E^+, h \cup B \models e$ and $\forall e \in E^-, h \cup B \not\models e$.
% \end{definition}


% \noindent
% We assume that $B$ contains the necessary language bias, such as mode declarations \cite{progol}, to define the hypothesis space $\mathcal{H}_{B}$, the set of all hypotheses (logic programs).
% % \noindent
% The ILP problem is to find a \emph{solution}:




% \begin{example}[Abstraction fold]


% \subsection{Abstraction and Instantiation}
% \label{sec:abs}
% \ch{need better motivation wrt the ilp problem}

% % \ac{@SD, this section is a shitshow. Any suggestions?}

% The higher-order refactoring problem takes as input a set of first-order clauses and a set of higher-order abstractions. We define an higher-order abstraction:
% % , (ii) higher-order abstractions, and (iii) support clauses.
% % We define (ii) and (iii) in turn.

% % \ac{explain why we need this definition}
% % We first definite a \emph{higher-order abstraction}.
% % \cite{metaho}:

% \begin{definition}[\textbf{Higher-order abstraction}]
% A \emph{higher-order abstraction} is a set of higher-order Horn clauses with the same head predicate symbol and arity.

% % that contain at least one atom which takes a predicate symbol an argument.
% \end{definition}

% \begin{example}
% The following program is the abstraction \emph{fold}:
% \begin{center}
% \begin{tabular}{l}
% \emph{fold(A,B,P,Q) $\leftarrow$ empty(A),P(B)}\\
% \emph{fold(A,B,P,Q) $\leftarrow$ head(A,C),tail(A,D),fold(D,E,P,Q),Q(C,E,B)}\\
% \end{tabular}
% \end{center}
% \end{example}

% \noindent
% To use higher-order abstractions, we need  \emph{support clauses} \cite{knorf}.
% \ch{not clear what support clauses are}
% \ch{I am confused, are support clauses from the Knorf paper rather equivalent to our candidates abstraction? if so, do we need both support clauses and candidate abstractions in definitions 2 and 4?}
% To illustrate the need for support clauses, suppose we have the rule:
% \begin{center}
% \emph{f(A,B) $\leftarrow$ tail(A,C),f(C,B)}
% \end{center}
% Then one higher-order abstraction of this rule is:
% \begin{center}
% \emph{inv(A,B,P) $\leftarrow$ P(A,C),inv(C,B,P)}
% \end{center}
% To redefine \emph{f} in terms of \emph{inv} we need to introduce a support clause of the form:
% \begin{center}
% \emph{f(A,B) $\leftarrow$ inv(A,B,tail)}
% \end{center}

\noindent
% We want to introduce higher-order abstractions to improve the performance of ILP system.
% The set of predicate symbols $T$ in Definition \ref{def:prob} 
% .
% \sd{Our explanation of replacing predicate in clauses might be confusing. We do this technically but conceptually we introduce new higher-order definition that is based on the existing definition, and rewrite the old definition by instantiating the new ho clause.}
We want to introduce higher-order abstractions that compress a logic program.
The idea of an abstraction is to replace a predicate symbol in the body of a definition with a predicate variable and add this variable to the head of the definition.
We define an abstraction:
% \begin{definition}[\textbf{Abstraction (V1)}]
% Let $r = h(t_1, t_2, \dots, t_k) \leftarrow b(s_1, s_2, \dots, s_m)$ be a first-order rule.
% Then $h(t_1, t_2, \dots, t_k, P) \leftarrow P(s_1, s_2, \dots, s_m)$ is a higher-order abstraction of $r$, where $P$ is a higher-order variable \ac{crap first try}.
% \end{definition}

\newcommand\mydots{\makebox[1em][c]{.\hfil.\hfil.}}

% \sd{this definition is really difficult to parse. simple fragmenting might help.}

% \sd{
% \begin{definition}[\textbf{Abstraction}]
% Let $P$ be a logic program. 
% Let
% $d \in D(P)$ be a definition with head predicate symbol $h$.
% Let $p$ be a predicate symbol in the body of a rule in $d$.
% Let $a$ be the program obtained by copying $d$ and replacing every instance of $p$ by a higher-order variable $V$, every occurrence of $h$ by an invented predicate \emph{ho}, and by adding $V$ to the arguments of literals with predicate \emph{ho}. 
% Then $a$ is an abstraction of $d$.
% % which abstracts away $p$.
% \end{definition}
% }

% \begin{definition}[\textbf{Abstraction}]
% Let $P$ be a logic program,
% $d \in D(P)$ be a definition with the head predicate symbol $h$,
% and $p$ be a predicate symbol in the body of a rule in $d$.
% Let 
% \emph{ho} be an invented predicate symbol not in $P$,
% $V$ be a higher-order variable,
% and $a$ be the definition obtained from $d$ by replacing every instance of $p$ by $V$, every instance of $h$ by \emph{ho}, and by adding $V$ to the arguments of literals with predicate $q$. 
% Then $a$ is an abstraction of $d$.
% % which abstracts away $p$.
% \label{def:abs}
% \end{definition}
% \noindent

% \begin{definition}[\textbf{Abstraction} (NEW)]
% Let $P$ be a logic program, 
% $d \in D(P)$ be a definition with the head predicate symbol $h$,
% and $p_1,\dots, p_n$ be a subset of the predicate symbols in the body of a rule in $d$.
% Let  \emph{ho} be an invented predicate symbol not in $P$,
% $V_1, \dots, V_n$ be higher-order variables,
% and $a$ be the definition obtained from $d$ by replacing every instance of $p_i$ by $V_i$, every instance of $h$ by \emph{ho}, and by adding $V_1, \dots, V_n$ to the arguments of literals with the predicate symbol $h$. 
% Then $a$ is an abstraction of $d$.
% % which abstracts away $p$.
% \label{def:abs}
% \end{definition}

\begin{definition}[\textbf{Abstraction and Instantiation}]
Let $P$ be a logic program, 
$d \in D(P)$ be a definition with the head predicate symbol $h$ of arity $k$,
and $p_1,\dots, p_n$ be a subset of the predicate symbols in the body of a rule in $d$.
Let  $h'$ be an invented predicate symbol not in $P$,
$x_1, \dots, x_n$ be higher-order variables,
and $a$ be the definition obtained from $d$ by 
(i) replacing every instance of $p_i$ with $x_i$, 
(ii) replacing every instance of $h$ with $h'$, 
and (iii) adding $x_1, \dots, x_n$ to the arguments of literals with the predicate symbol $h$. 
Then $a$ is an \emph{abstraction} of $d$.
Let $v_1, ..., v_k$ be first-order variables. 
Then the rule $h(v_1, ..., v_k) \leftarrow h'(v_1, ..., v_k, p_1, \dots, p_n)$ is an \emph{instantiation} of $a$.
% which abstracts away $p$.
\label{def:abs}
\end{definition}

\noindent
We denote invented predicate symbols ($h'$ in the above definition) with the prefix \emph{ho}.
% inv \ch{is 'abs' better?}.
% \begin{definition}[\textbf{Abstraction}]
% Let 
% $D$ be a definition, $r = h(t_1, \dots, t_a) \leftarrow b_1, \dots, b_n$ be a rule in $P$,
% $p_i(x_1, \dots, x_k)$  be a non-recursive body literal $i$ of $r$,
% $p_i$ be a predicate symbol, 
% $C = aux_h(t_1, \mydots, t_a, P) \leftarrow b_1, \mydots b_{i-1}, b_{i+1}, \mydots, b_n, P(x_1, \mydots, x_k)$, 
% $D = h(t_1, \mydots, t_a) \leftarrow aux_h(t_1, \mydots, t_a, p_i)$, 
% $P$ be a predicate variable,
% and $aux_h$ be a new predicate symbol not in $P$.
% Then the set $\{C,D\}$ is an \emph{abstraction} of $r$.
% \end{definition}

% \ac{give an example}
% \ac{give an example of an abstraction on an already abstracted rule}
% \ac{unclear what a `new invented symbol is`}

% \ac{the above is crap}
% \begin{definition}[same as above but for definitions (recursive programs)]
% \ac{TODO}
% \end{definition}

% \begin{definition}[same as above but for logic programs]
% \ac{TODO}
% \end{definition}

% \begin{definition}[\textbf{Instantiation}]
% Let $r$ be a rule with the head literal $p(t_1, \mydots, t_a)$ and $r'$ be an abstraction of $r$ with the head literal 
% $a_r(t_1, \mydots, t_a, P)$.

% Then an instanstiation of r' and a' is the rule $p(t_1, \dots, t_a) \leftarrow a_r(t_1, \dots, t_a, p_i)$.

% \ac{TODO}
% \end{definition}

% \ch{how about a definition along those lines?}
% \ch{simply trying to break down the definition, very messy}
% \begin{definition}[\textbf{Abstraction of a literal}]
% Let $l=p(a_0, ..., a_a)$ be a literal with predicate symbol $p$ and arity $a$, $p_{aux}$ a new predicate symbol, $V$ a higher-order variable. The abstraction of $l$ is the literal $A_{p_{aux}, V}(l) = p_{aux}(a_0, ..., a_a,V)$.
% \end{definition}

% \begin{definition}[\textbf{Abstraction}]
% Let $P$ be a first-order definition defining the relation $p$ of arity $a$, $q$ a predicate symbol, $V$ a higher-order variable, $p_{aux}$ a new predicate symbol. An abstraction of $P$ is a higher-order program $A_{q,p_{aux},V}(P)=\{P', Q\}$
% where $P'$ is obtained by abstracting the literals with predicate symbol $p$ $A_{p_{aux}, V}$ in $P$ and subtituting $q$ by $V$, and $Q = \{p(a_0, ..., a_a)\} \leftarrow p_{aux}(a_0, ..., a_a,q)\}$ where $a_0, ..., a_a$ are first-order variables.
% % \ch{very messy, not sure about the added arguments}
% \end{definition}

\begin{myexample}[\textbf{Abstraction}]
\label{ex:abs}
Consider the rule:
\[
\begin{tabular}{l}
    \emph{f(A) $\leftarrow$ head(A,B),one(B),tail(A,C),head(C,D),one(D)}
    \end{tabular}
\]
One abstraction of this rule is:
\[
% a_1 = \left\{
\begin{tabular}{l}
    % \emph{f(A) $\leftarrow$ inv1(A,one)}\\
 \emph{ho$_1$(A,P) $\leftarrow$ head(A,B),P(B),tail(A,C),head(C,D),P(D)}
\end{tabular}
    % \right\}
\]
Another abstraction is:
\[
% a_1 = \left\{
\begin{tabular}{l}
    % \emph{f(A) $\leftarrow$ inv1(A,one)}\\
 \emph{ho$_2$(A,P) $\leftarrow$ head(A,B),one(B),P(A,C),head(C,D),one(D)}
\end{tabular}
    % \right\}
\]

% Consider the rule:
% \[
% \begin{tabular}{l}
%     \emph{f(A,P) $\leftarrow$ head(A,B),P(B),tail(A,C),head(C,D),P(D)}
% \\
%     \end{tabular}
% \]
\noindent
% One abstraction of this \emph{ho$_1$} rule is:
% \[
% \begin{tabular}{l}
%  \emph{ho$_2$(A,P,Q) $\leftarrow$ Q(A,B),P(B),tail(A,C),Q(C,D),P(D)}
%     \end{tabular}
% \]
Consider the definition:
\[
\begin{tabular}{l}
    \emph{f(A) $\leftarrow$ head(A,B),one(B)}\\
    \emph{f(A) $\leftarrow$ tail(A,B),f(B)}
\\
    \end{tabular}
\]
One abstraction of this definition is:
\[
\begin{tabular}{l}
    \emph{ho(A,P) $\leftarrow$ head(A,B),P(B)}\\
    \emph{ho(A,P) $\leftarrow$ tail(A,B),ho(B,P)}
    \end{tabular}
\]
% Consider the following program:
% \[
% \begin{tabular}{l}
%     \emph{f(A) $\leftarrow$ head(A,B),one(B)}\\
%     \emph{f(A) $\leftarrow$ tail(A,B),f(B)}
%     \end{tabular}
% \]
% Then one higher-order abstraction of this program is:
% \[
% \begin{tabular}{l}
%     \emph{f(A,P) $\leftarrow$ inv3(A,one)}\\
%  \emph{inv3(A,P) $\leftarrow$ head(A,B),P(B)}\\
%  \emph{inv3(A,P) $\leftarrow$ tail(A,B),inv3(B,P)}
%     \end{tabular}
% \]
\end{myexample}

% \begin{definition}[\textbf{Abstraction space}]
% Let $P$ be a logic program
% % $d \in D(P)$ be a definition,
% and 
% $a(d)$ be the set of all abstractions of the definition $d$, 
% % and $a^i$ be the $i^{th}$ functional power of $a$ ($i^{th}$ functional power can be defined inductively by $a^n = a \circ a^{n-1} = a^{n-1} \circ a$).
% % abstraction operator 
% Then the \emph{abstraction space} ${\cal{A}}(P)$ is the set of all abstractions of $P$:

% $${\cal{A}}(P) = \bigcup_{d\in D(P), i>0} a^i(d)$$ 
% % \ac{todo, generalise over all D}
% \end{definition}


% \begin{definition}[\textbf{Abstraction space NEW1}]
% Let $P$ be a logic program
% and 
% $a(d)$ be the set of all abstractions of the definition $d$. 
% % abstraction operator 
% Then the \emph{abstraction space} ${\cal{A}}_{0}(P)$ is the set of all abstractions of $P$:
% $${\cal{A}}_{0}(P) = \bigcup_{d\in D(P)} a(d)$$ 
% % \ac{todo, generalise over all D}
% \end{definition}

% \begin{definition}[\textbf{Abstraction space NEW2}]
% Let $P$ be a logic program
% and 
% $a(d)$ be the set of all abstractions of the definition $d$. 
% % abstraction operator 
% Then the \emph{abstraction space} ${\cal{A}}_{i+1}(P)$ is the set of all abstractions of $P$:
% $${\cal{A}}_{i+1}(P) =  
% {\cal{A}}_{i}(P) \bigcup_{d\in D({\cal{A}}_{i}(P))} a(d)$$ 
% % \ac{todo, generalise over all D}
% \end{definition}

% \ch{I think it is best to focus on simple abstractions up to this point, and start talking about abstractions of abstractions from here}
% \ch{introduce the idea of absractions of abstracions} 
% \sd{I like this focus on single predicate and then doing a fix-point iteration.}

\noindent
An abstraction replaces a single predicate symbol in a definition with a higher-order variable.
To replace more than one predicate symbol, we introduce the abstraction space:
\begin{definition}[\textbf{Abstraction space}]
Let $P$ be a logic program
and 
$\alpha(d)$ be the set of all abstractions of the definition $d$.
Then the \emph{abstraction space} ${\cal{A}}_{j}(P)$ for $j\geq 0$ of $P$ is:
\begin{align*} 
{\cal{A}}_{0}(P) &= P \\
{\cal{A}}_{i+1}(P) &=  
{\cal{A}}_{i}(P) \bigcup_{d\in D({\cal{A}}_{i}(P))} \alpha(d)\\
\end{align*} 
\end{definition}
% \ac{we can prove that this space/operator reaches a fixed point, as there as only finitely many body predicate symbols to remove. We can then refer to this fixed point set in subsequent definitions}
\begin{myexample}[\textbf{Abstraction space}]
\label{exabstraction}
Consider the program:
\begin{center}
\begin{tabular}{l}
$P$ = 
\left\{
    \begin{tabular}{l}
\emph{f(A,B) $\leftarrow$ tail(A,C),tail(C,D),head(D,B)}
    \end{tabular}
     \right\}
\end{tabular}
\end{center}
The abstraction space of $P$ is: 
\begin{center}
\begin{tabular}{l}
$\mathcal{A}_1(P)$ = 
$\mathcal{A}_0(P) \cup$ \\
\[ \left\{
    \begin{tabular}{l}
    \emph{ho$_1$(A,B,P) $\leftarrow$ P(A,C),P(C,D),head(D,B)}\\
    \emph{ho$_2$(A,B,P) $\leftarrow$ tail(A,C),tail(C,D),P(D,B)}\\
    \end{tabular}
     \right\}
\]\\


% \begin{align*} 
% {\cal{A}}_{2}(P) &=  {\cal{A}}_{1}(P) cup
% {\cal{A}}_{i}(P) \bigcup_{d\in D({\cal{A}}_{i}(P))} \alpha(d)\\
% \end{align*} 

$\mathcal{A}_2(P)$ = 
$\mathcal{A}_1(P) \cup$ \\
\[ \left\{
    \begin{tabular}{l}
    \emph{ho$_3$(A,B,P,Q) $\leftarrow$ P(A,C),P(C,D),Q(D,B)}\\    
    \end{tabular}
     \right\}
\]
\end{tabular}
\end{center}
\ac{sad syntax}
\end{myexample}

\begin{myexample}[\textbf{Abstraction}]
Consider the recursive definition:
\begin{center}
\begin{tabular}{l}
\emph{f(A,B) $\leftarrow$ head(A,B)}\\
\emph{f(A,B) $\leftarrow$ tail(A,C),f(C,B)}
\end{tabular}
\end{center}
The abstraction space of this definition is the set:
% \begin{center}
\[ \left\{
    \begin{tabular}{l}
\emph{ho$_4$(A,B,P) $\leftarrow$ P(A,B)}\\
\emph{ho$_4$(A,B,P) $\leftarrow$ tail(A,C),ho$_4$(C,B,P)}
    \end{tabular}
     \right\}
\] 
\[
    \left\{
    \begin{tabular}{l}
\emph{ho$_5$(A,B,P) $\leftarrow$ head(A,B)}\\
\emph{ho$_5$(A,B,P) $\leftarrow$ P(A,C),ho$_5$(C,B,P)}
    \end{tabular}
     \right\}
  \] 
\[   
    \left\{
    \begin{tabular}{l}
\emph{ho$_6$(A,B,P,Q) $\leftarrow$ P(A,B)}\\
\emph{ho$_6$(A,B,P,Q) $\leftarrow$ Q(A,C),ho$_6$(C,B,P,Q)}
    \end{tabular}
     \right\}
\]
\end{myexample}

% \left\{
%     \begin{tabular}{l}
%     \emph{ho$_3$(A,B,P,Q) $\leftarrow$ P(A,C),P(C,D),Q(D,B)}\\
%     \end{tabular}
%      \right\}
% \begin{myexample}[\textbf{Abstraction}]
% \label{ex:abs}
% Consider the rule:
% \[
% \begin{tabular}{l}
%     \emph{f(A) $\leftarrow$ head(A,B),one(B),tail(A,C),head(C,D),one(D)}
%     \end{tabular}
% \]
% One abstraction of this rule is:
% \[
% % a_1 = \left\{
% \begin{tabular}{l}
%     % \emph{f(A) $\leftarrow$ inv1(A,one)}\\
%  \emph{ho$_1$(A,P) $\leftarrow$ head(A,B),P(B),tail(A,C),head(C,D),P(D)}
% \end{tabular}
%     % \right\}
% \]
% Another abstraction is:
% \[
% % a_1 = \left\{
% \begin{tabular}{l}
%     % \emph{f(A) $\leftarrow$ inv1(A,one)}\\
%  \emph{ho$_2$(A,P) $\leftarrow$ head(A,B),one(B),P(A,C),head(C,D),one(D)}
% \end{tabular}
%     % \right\}
% \]
% \end{myexample}
\noindent
\ac{an abstraction blah blah blah}
An instantiation replaces a predicate variable in an abstraction with a predicate symbol:
\begin{definition}[\textbf{Instantiation space NEW}]
Let $P$ be a logic program,
$\mathcal{A}(P)$ be the abstraction space of $P$,
$p$ be a head predicate symbol in $P$ with arity $m$,
$q$ be a head predicate symbol in $\mathcal{A}P$ with arity $n$,
and $v_1, ..., v_k$ be first-order variables. 
Then the rule $h(v_1, ..., v_k) \leftarrow h'(v_1, ..., v_k, p)$ is an \emph{instantiation} of $a$.
% with $p$. 
% \ch{what is the domain of $p$?}
\end{definition}

\begin{definition}[\textbf{Instantiation}]
Let $P$ be a logic program,
$d \in D(P)$ be a definition with the head predicate symbol $h$ of arity $k$, 
$a \in \alpha(d)$ be an abstraction of $d$ with head predicate symbol $h'$, 
$p$ be a predicate symbol in $P$, 
and $v_1, ..., v_k$ be first-order variables. 
Then the rule $h(v_1, ..., v_k) \leftarrow h'(v_1, ..., v_k, p)$ is an \emph{instantiation} of $a$.
% with $p$. 
% \ch{what is the domain of $p$?}
\end{definition}

% \begin{definition}[\textbf{Instantiation}]
% Let $P$ be a logic program,
% $\mathcal{A}(P)$ be the abstraction space of $P$,
% $h$,
% % of arity $k$, 
% % $a \in A(d)$ be an abstraction of $d$ with head predicate symbol $h'$, 
% Let $p$ be a predicate symbol in $P$ and $v_1, ..., v_k$ be first-order variables. 
% Then the rule $h(v_1, ..., v_k) \leftarrow h'(v_1, ..., v_k, p)$ is an \emph{instantiation} of $a$.
% % with $p$. 
% % \ch{what is the domain of $p$?}
% \end{definition}


\begin{myexample}[\textbf{Instantiation}]
Consider the abstractions from Example \ref{ex:abs}.
One instantiation of \emph{ho$_2$} is:
\begin{center}
\begin{tabular}{l}
\emph{f(A,B) $\leftarrow$ ho2(A,B,head)}
\end{tabular}
\end{center}
% One instantiation of \emph{ho$_3$} is:
% \begin{center}
% \begin{tabular}{l}
% \emph{ho2(A,B,P) $\leftarrow$ ho3(A,B,P,tail)}
% \end{tabular}
% \end{center}
\end{myexample}



% \begin{definition}[\textbf{Abstraction space NEW CH}]
% Let $P$ be a logic program
% and 
% $A(d)$ be the set of all abstractions of the definition $d$.
% Then the \emph{abstraction space ${\cal{A}}_{i}(P)$ of level $i$} of $P$ is:
% % \[
% %     \begin{array}{l}
% % {\cal{A}}_{0}(P) = \bigcup_{d\in D(P)} a(d)\\
% % {\cal{A}}_{i+1}(P) =  
% % {\cal{A}}_{i}(P) \bigcup_{d\in D({\cal{A}}_{i}(P))} a(d)\\
% %     \end{array}
% % \]
% % \begin{equation*} \label{eq1}
% % \begin{split}
% \begin{align*} 
% {\cal{A}}_{1}(P) &= \bigcup_{d\in D(P)} A(d)\\
% \forall i \geq 1, {\cal{A}}_{i+1}(P) &= \bigcup_{d\in D({\cal{A}}_{i}(P))} A(d)
% \end{align*} 
% % \end{split}
% % \end{equation*}
% % \begin{tabular}{l}
% %      $${\cal{A}}_{0}(P) = \bigcup_{d\in D(P)} a(d)$$\\
% %     $${\cal{A}}_{i+1}(P) =  
% % {\cal{A}}_{i}(P) \bigcup_{d\in D({\cal{A}}_{i}(P))} a(d)$$
% % \end{tabular}
% The \emph{abstraction space} of $P$ is:
% \begin{align*} 
% {\cal{A}}(P) &= \bigcup_{i \geq 1}  {\cal{A}}_{i}(P)
% \end{align*} 
% \end{definition}

\noindent
% We define the abstraction space:


\noindent
% \ac{The idea of an instantiation is to ...
% } 


\noindent
We define the instantiation space:
\begin{definition}[\textbf{Instantiation space}]
% \ac{The instantiation space I(A(P)) of the logic program $P$ is ...}
Let $P$ be a logic program, and $I(A(P))$ the set of instantiations of the abstractions $A(P)$. The instantiation space for $i \geq 1$ of $P$ is:
\begin{align*} 
{\cal{I}}_{1}(P) &= I(A(P)) \\
{\cal{I}}_{i+1}(P) &=  
{\cal{I}}_{i}(P) \bigcup_{d\in D({\cal{A}}_{i}(P))} I(A(d))\\
\end{align*} 
% The instantiation space ${\cal{I}}({\cal{A}}(P))$ of the logic program $P$ is the set of all instantiations of all abstractions in the abstraction space of $P$.
% \ch{the previous definition only defines instantiations of level 1, while we talk about the abstraction space here}
\end{definition}

% \ac{
% We cannot derive $f(A) \leftarrow inv2(A,one,head)$ with my rubbish definition. 
% My definiton also does not work with recursive rules.
% }
\noindent
% \ac{the idea of ....}
The idea of refactoring is to introduce abstractions and instantiations to compress a program.
When we refactor a program, we want to preserve its semantics.
However, we only need to preserve the semantics with respect to a subset of the predicates, namely the head predicate symbol.
Therefore, we reason about the least Herbrand model restricted to a set of predicate symbols:
\begin{definition}[\textbf{Restricted least Herbrand model}]
Let $P$ be a logic program, $M(P)$ be the least Herbrand model of $P$, 
and $T$ be a set of predicate symbols.
Then the least Herbrand model of $P$ restricted to $T$ is $M_T(P) = \{ a \in M(P) \,|\, \text{the predicate symbol of $a$ is in } T\}$.
\end{definition}

% \noindent
% We show that an instantiation of an abstraction preserves the restricted least Herbrand model semantics of the logic program restricted to the head predicate symbol:
% \begin{proposition}
% Let $d$ be a definition with head predicate symbol $h$, $p$ be a predicate symbol in the body of a
% rule in $d$, $a \in {\cal{A}}(D)$ the abstraction which abstracts away the predicate $p$, and $i \in {\cal{I}}({\cal{A}}(D)$ the instantiation of $a$ with $p$. \ch{rather A(D)?}
% Then $M_h(d) == M_h(a \cup i)$.
% \label{semantics}
% \end{proposition}
% \begin{proof}
% The proof is in the appendix and follows from the results by Cropper and Tourret \shortcite{reduce}.
% \end{proof}

% \begin{proposition}
% Let $P$ be a first-order program, $A$ be an abstraction of $P$, and $T$ be a set of the head predicate symbols of $P$.
% Then $M_T(A) == M_T(P)$.
% \end{proposition}
% \begin{proof}
% \ac{The proof is in the appendix and follows from the results by \citet{reduce}.}
% \end{proof}

% \noindent

% \ac{@AC, an example here would help}.

% We focus on success set equivalence. \cite{maher?}.
% The success set $SS(P)$ of a logic program $P$ is the set of ground atoms from the Herbrand base of $P$ which have a successful SLD-derivation for $P$ .
% The success set of a logic program \emph{P} is the set of ground atoms $\{ a \in hb(P)|P \cup \{ \neg a \}$ has a SLD-refutation\}, where \emph{hb(P)} represents the Herband base of the logic program \emph{P}.

% The suc- cess set restricted to a specific predicate symbol p is the subset of the success set restricted to atoms containing the predicate symbol p.

% We define a specific instance of the refactoring problem \cite{knorf}.
% In this problem,  where the goal is to refactor the BK ....

% \begin{definition}[\textbf{Success set}]
% % SS(p, P ) = {α ∈ SS(P )|α has predicate symbol p}
% \end{definition}
% the success set of $P$ restricted to the symbols in $T$.


% \noindent
% We define the \emph{higher-order refactoring} input:
% \begin{definition}[\textbf{Higher-order refactoring input}]
% \label{def:input}
% A higher-order refactoring input is a tuple ($P$, $A$, $T$) where 
% $P$ is a first-order definite program, 
% $A$ is a higher-order program, and $T$ is a set of predicate symbols.
% % , and $S$ is a set of support clauses.
% \end{definition}
% \noindent

% \ac{@AC, clarify what this statement means: The higher-order program $A$ is a set of candidate abstractions.}
% \sd{A stands for the candidate high-order programs?}
% \ch{yes}
% \ac{@AC, why T?}
% \noindent

% \subsection{Higher-Order Refactoring Problem}
% \label{sec:hoprob}
\noindent
We define the \emph{higher-order refactoring} problem:

\begin{definition}[\textbf{Higher-order refactoring problem}]
\label{def:prob}
Let $P$ be a logic program and $T$ be a set of predicate symbols.
Then the \emph{higher-order refactoring problem} is to find $Q \subseteq {\cal{A}}(P) \cup {\cal{I}}({\cal{A}}(P))$ such that $M_T(Q) == M_T(P)$.
We call $Q$ a \emph{solution} to the refactoring problem.
\end{definition}


% \begin{definition}[\textbf{Higher-order refactoring problem}]
% \label{def:prob}
% Given a logic program P, the 
% Let ($P$, $A$, $T$) be a higher-order refactoring input. 
% Then the \emph{refactoring problem} is to find $Q \subset P \cup A$ such that $M_T(Q) == M_T(P)$.
% We call $Q$ a \emph{solution} to the refactoring problem.
% \end{definition}

\noindent
Our goal is to perform \emph{optimal refactoring}:
% \begin{definition}[\textbf{Optimal refactoring}]\label{def:opti}
% Let ($P$, $A$, $T$) be a higher-order refactoring input and \emph{size}
% % : $\mathcal{H} \mapsto \mathbb{N}$
% be a function that measures the size of a logic program.
% Then $Q$ is an \emph{optimal} solution to the refactoring problem when (i) $Q$ is a solution to the refactoring problem, and (ii) there is no $Q' \subset P \cup A$ such that $Q'$ is a solution to the refactoring problem and $size(Q') < size(Q)$.
% \end{definition}


\begin{definition}[\textbf{Optimal refactoring}]\label{def:opti}
Let $P$ be a logic program and $T$ be a set predicate symbols.
Then $Q$ is an \emph{optimal} solution when (i) $Q$ is a solution to the refactoring problem, and (ii) there is no $Q' \subseteq {\cal{A}}(P) \cup {\cal{I}}({\cal{A}}(P))$ such that $Q'$ is a solution to the refactoring problem and $size(Q') < size(Q)$.
\end{definition}


% Then the \emph{higher-order refactoring problem} is to find $Q \subset P \cup A(P)$ such that $M_T(Q) == M_T(P)$.
% We call $Q$ a \emph{solution} to the refactoring problem.


% \begin{equation}
% \arg \min_{k} P(k)
% \end{equation}

    \noindent
In the next section, we introduce \name{}, which solves the refactoring problem by formulating it as a COP.
% \subsection{Support Clauses}
% We refactor a logic program by abstracting and then compressing it.

% We refer the reader to the work of \citeauthor{knorf} (\citeyear{knorf}) for more details on support clause
% \ac{more here?}



% \noindent
% Even if we assume that the refactoring problem is decidable, optimal refactoring is NP-hard:

% \begin{theorem}[\textbf{Optimal refactoring complexity}]
% \label{thm:nphard}
% Optimal refactoring is NP-Hard.
% \end{theorem}
% \begin{proof}
% We can reduce the knapsack problem, which is NP-Hard, to optimal refactoring.
% \end{proof}

% \subsection{ILP Problem Complexity}

% \subsection{Sample Complexity Reduction}
% \label{sec:sampcomp}
% To explain why refactoring can improve learning performance, we formalise the impact of refactoring on Metagol \cite{mugg:metagold,metagol}, a state-of-the-art ILP system, which we use in our experiments.
% Metagol takes as input (1) positive and negative examples (ground atoms) of a target concept, (2) BK, and (3) a set of \emph{metarules}, higher-order Horn clauses to restrict the form of hypotheses.
%  % \cite{crop:reduce}.
% These inputs define the Metagol hypothesis space which in turn determines its sample complexity \cite{metaho}:

% \begin{proposition}[\textbf{Sample complexity}]
% \label{prop:sampcomp}
% Let $m$ be the number of metarules with at most $j$ body literals, $p$ be the number of predicate symbols in the BK, and $n$ be the minimal number of clauses need to express the target hypothesis given the BK.
% Then with error $\epsilon$ and confidence $\delta$ Metagol has sample complexity
% $s \geq \frac{1}{\epsilon} (n \ln(m) + (j+1)n \ln(p) + \ln\frac{1}{\delta})$.
% \end{proposition}

% % \noindent
% % The authors use this result to calculate the Metagol sample complexity:

% % \begin{proposition}[\textbf{Sample complexity}]
% % \label{prop:sampcomp}
% % With error $\epsilon$ and confidence $\delta$ MIL has sample complexity
% % $s \geq \frac{1}{\epsilon} (n \ln(m) + (j+1)n \ln(p) + \ln\frac{1}{\delta})$.
% % \end{proposition}


% \noindent
% % According to the Blumer bound \cite{behw-or-87}, given two hypothesis spaces of different sizes, searching the smaller space will result in fewer errors, assuming that the target hypothesis is in both spaces.
% If we assume (1) a fixed set of metarules, and (2) that we do not exclude the target hypothesis, then Proposition \ref{prop:sampcomp} shows that we can reduce the Metagol sample complexity by either reducing the number of predicate symbols $p$ or the size of the target program $n$.
% We can reduce $p$ by compressing the BK:

% \begin{theorem}[\textbf{Branching reduction}]
% \label{thm:branchreduce}
% Suppose that refactoring can reduce the number of predicate symbols from $p$ to $p'$.
%  % and let $r = p'/p$ be the reduction ratio.
% Then refactoring reduces the Metagol sample complexity by $(p'/p)^{j+1}$.
% \end{theorem}
% \begin{proof}
% Replacing $p$ with $p'/p$ in Proposition \ref{prop:sampcomp} and rearranging terms leads to
% $s \geq \frac{1}{\epsilon} (n \ln(m) + (j+1)n \ln(p'/p) + (j+1)n \ln(p) + \ln\frac{1}{\delta})$.
% \end{proof}

% \noindent
% Likewise, we can reduce $n$ by refactoring the BK so that we can express the target hypothesis with fewer clauses:

% \begin{theorem}[\textbf{Depth reduction}]
% \label{thm:depthreduce}
% Suppose that refactoring can reduce the number of clauses needed to express a target theory from $n$ to $n'$.
% Then refactoring reduces the Metagol sample complexity by $(j+1)(n-n') \ln(p)$.
% \end{theorem}
% \begin{proof}
% \ac{todo}
% \end{proof}

% \noindent
% Theorems \ref{thm:branchreduce} and \ref{thm:depthreduce} show that refactoring can substantially reduce the sample complexity of Metagol.
% \ac{Note that these results should generalise to other ILP approaches.}


% \subsection{Benefit of Refactoring}
% To show the potential benefits of refactoring, imagine an ILP system that enumerates all programs in the hypothesis space, a common approach when inducing functional programs ~\cite{deepcoder,dreamcoder}.
% We adapt the result of \citet{popper} to calculate the size of the hypothesis space:

% \begin{proposition}[\textbf{Hypothesis space size}]
% \label{prop:hspace}
% Let $p$ be the number of predicate symbols allowed in a hypothesis, $m$ be the maximal number of literals in a clause in a hypothesis, $v$ be the maximum number of unique variables in a hypothesis, and $n$ be the maximum number of clauses in a hypothesis.
% Also assume, for simplicity, that the arity of each predicate is $a$.
% Then the maximum number of hypotheses in the hypothesis space is
% % \[\sum_{j=1}^n {\sum_{i=1}^m {pv^a \choose i} \choose j} \]
% $\sum_{j=1}^n {\sum_{i=1}^m {pv^a \choose i} \choose j}$.
% \end{proposition}
% \begin{proof}
% Let $C$ be an arbitrary clause in the hypothesis space.
% There are $pv^a$ ways to define a literal in $C$.
% $C$ is a set of literals.
% There are $pv^a \choose k$ ways to choose $k$ literals.
% We bound the number of body literals to $m$, so there are $\sum_{i=1}^m {pv^a \choose i}$ ways to choose at most $m$ literals and, therefore, to define $C$.
% A hypothesis is a set of definite clauses.
% Given $n$ clauses, there are $n \choose k$ ways to choose $k$ clauses to form a hypothesis.
% Therefore, there are $\sum_{j=1}^n {\sum_{i=1}^m {pv^a \choose i} \choose j}$ ways to define a hypothesis with at most $n$ clauses.
% \end{proof}

% \noindent
% According to the Blumer bound \cite{blumer:bound}, given two hypothesis spaces of different sizes, and assuming that the target hypothesis is in both spaces, searching the smaller space will result in fewer errors compared to the larger one.
% This result implies that we can improve the performance of an ILP system by either reducing the number of predicate symbols $p$ or the size of the target program $n$.
% By refactoring we can reduce $p$ by removing redundant predicate symbols and also by limiting the number of predicate symbols allowed in the BK.
% We can also reduce $m$ and $n$ by restructuring the BK so that we can express the target hypothesis (program) using shorter ($m$) or fewer $n$ clauses.
% % We argue that refactoring is especially important in a \emph{lifelong learning} setting where a system continuously learns thousands of new concepts, i.e. where $p$ can be enormous.




